Bhasha-Abhijnaanam: Native-script and romanized Language Identification for 22 Indic languages

We create publicly available language identification (LID) datasets and models in all 22 Indian languages listed in the Indian constitution in both native-script and romanized text. First, we create Bhasha-Abhijnaanam, a language identification test set for native-script as well as romanized text which spans all 22 Indic languages. We also train IndicLID, a language identifier for all the above-mentioned languages in both native and romanized script. For native-script text, it has better language coverage than existing LIDs and is competitive or better than other LIDs. IndicLID is the first LID for romanized text in Indian languages. Two major challenges for romanized text LID are the lack of training data and low-LID performance when languages are similar. We provide simple and effective solutions to these problems. In general, there has been limited work on romanized text in any language, and our findings are relevant to other languages that need romanized language identification. Our models are publicly available at https://ai4bharat.iitm.ac.in/indiclid under open-source licenses. Our training and test sets are also publicly available at https://ai4bharat.iitm.ac.in/bhasha-abhijnaanam under open-source licenses.

==> LID.tex <==
\section{Introduction}
\textbf{Importance of languageID in general./ Application of LanguageID in general} \\
Language identification is an important task in natural language processing and computational linguistics. It is the process of automatically determining the language of a given piece of text, and it is often used as a preprocessing step in a number of applications, such as machine translation, information retrieval, and sentiment analysis.
In machine translation, using language identification can improve the accuracy and fluency of the translated text by ensuring that the appropriate translation model is used for the language of the source text. In sentiment analysis, language identification can help to better interpret and understand the text and the emotions it conveys, leading to more accurate sentiment predictions. In web crawling, language identification can help to extract more accurate and relevant information from web pages, and can also be used to filter out pages that are not in the target languages. Additionally, the rules for grammar and syntax can vary between languages, which can affect the overall structure and coherence of the text, influencing the efficacy of the task at hand. Overall, language identification is important for enabling computers to understand and process human language, and by accurately identifying the language of a piece of text, the language identification model can enable other natural language processing tasks to be performed more accurately and effectively. \\
\textbf{Importance of languageID in web crawl/ Application of LanguageID in web crawl} \\
- read LangID in wild paper 

\textbf{Approaches in Language identification task}
There are various approaches to language identification, but the most common one is to use a machine learning model that has been trained on a large dataset of text in different languages. The model is trained to recognize the unique characteristics of each language, such as the frequency and distribution of different characters, words, and phrases. When the model is presented with a new piece of text, it uses this information to determine the most likely language that the text is written in. \\
\textbf{Challenges in Language identification task}
Language identification can be challenging because there are many languages in the world, and they can have similar characteristics that make them difficult to distinguish from one another. Additionally, some languages have dialects or variations that can make language identification even more difficult. However, with the right training data and machine learning model, it is possible to achieve high levels of accuracy in language identification.\\
\textbf{Importance of languageID in Indian languages more spicifically for roman inputs} \\
% The Indian subcontinent is home to diverse languages across four major language families written in multiple scripts \cite{daniels1996world}.
% In various settings such as in instant messaging, web search, and social media, these languages are commonly romanized owing to users' familiarity with the input tools for the Latin script.
% Often, there is large diversity in how words are romanized: For instance, even the short word \texthindi{मैं} (\textit{I}) can be romanised in multiple ways: \textit{main, mai, mein, mei} which overlap with the ways of romanising another short word, \texthindi{में} (\textit{in}). This widespread usage of romanization and lack of standardization implies that accurate transliteration models form a critical component in the NLP stack for Indian languages used by over 735 million Internet users \cite{KPMG-Report}.
% The Indian subcontinent is home to diverse languages spanning four major language families (Indo-Aryan branch of Indo-European, Dravidian, Austro-Asiatic, and Tibeto-Burman) spoken by more than a billion speakers. These languages are written in multiple scripts, including Abugida scripts from the Brahmi family, Arabic-derived abjad scripts, and alphabetic Roman scripts \cite{daniels1996world}. Creating user-friendly input tools is challenging due to the diverse nature of Indic languages and scripts. \\
% Indians and increasingly communicating online and engaging.  According to a study \cite{KPMG-Report} there are more than 735 million Internet users in India as of 2021, of which a large majority (536 million) prefer to communicate in their native language and 70\% of Indian language users identify challenges in using English keyboards.
% A large proportion of these non-English speakers access the Internet in their native languages but use the Roman script to express themselves through various communication channels like messages and posts. Romanized inputs has wide adoption among the population. 
The Indian subcontinent is home to a diverse range of languages spoken by over a billion people. These languages belong to four major language families: Indo-Aryan branch of Indo-European, Dravidian, Austro-Asiatic, and Tibeto-Burman. These languages are written using a variety of scripts, including Abugida scripts from the Brahmi family, Arabic-derived abjad scripts, and alphabetic Roman scripts.
As the use of the Internet grows in India, more and more people are using it to communicate in their native languages. According to a study, there are over 735 million Internet users in India as of 2021, and a large majority of these users (536 million) prefer to communicate in their native languages.
A significant proportion of these non-English speakers access the Internet in their native languages, but they use the Roman script to express themselves through various communication channels like messages and posts. The use of Romanized inputs is widespread among the population. 
% This highlights the need for accurate language identification in order to better understand and process the vast amounts of text in Indian languages that are written in Roman script.
Romanized input is commonly used in settings such as instant messaging, web search, and social media due to users' familiarity with the input tools for the Latin script. In these settings, it is common to see Indian languages written using the Roman script, as it allows users to easily input text using familiar keyboard layouts and input methods. This widespread use of Romanized input highlights the need for accurate language identification in order to better understand and process the vast amounts of text in Indian languages that are written in the Roman script. Accurate language identification can enable a wide range of applications and tools for text processing and analysis, and it is an important area of research and development in the field of natural language processing.\\
% \indent    - usage of roman inputs in general \\
% \indent    - why we need to identify the language of those roman inputs \\
\textbf{No train data is available and why it is important to generate the synthetic train data.} \\
There is no training data is available to train a language identification model for romanized input, one solution is to generate a training dataset using a transliteration model. A transliteration model is a type of machine learning model that is trained to convert text written in one script into another script. For example, a transliteration model could be trained to convert text written in the Devanagari script into Roman script. This generated Roman script text could then be used as training data for a language identification model.
The transliteration model would capture the full range of language characteristics. Once the transliteration model is trained, it can be used to generate Roman script text from the source script text, which can then be labeled with the corresponding language and used as training data for the language identification model.
By using a transliteration model to generate training data, it is possible to create a large and diverse dataset that can be used to train a language identification model for romanized input. This can help to improve the model's accuracy and enable it to handle a wide range of languages and scripts. Overall, using a transliteration model to generate training data can be an effective approach for developing a language identification model for romanized input.\\
\textbf{Our contributions} \\
In this work, we introduce a Roman language identification model for 20 Indian languages. This is the first model of its kind and has not been previously explored.
We also provide a benchmark test set for these 20 languages and evaluate our model using both the Dakshina roman test set and our new LID test set and establish baselines. 
% Our model is a two-stage approach that uses a combination of a lightweight fasttext model and a powerful IndicBERT model. This allows us to achieve both fast inference times and accurate predictions. 
Our proposed model is a two-stage approach that accepts inputs in 24 native scripts, 20 roman scripts, English, and other languages. The first stage uses a fasttext model, which is a light-weight model with a single linear layer that offers fast inference time. The second stage uses IndicBERT, which is a more powerful model with more parameters that is able to provide accurate predictions when the fasttext model fails. The combination of these two models offers the benefits of both in terms of inference time and prediction accuracy.
We also introduce a novel approach to generate synthetic romanized data using a transliteration model, which allows us to train our language identification model even when no training data is available. 
We also perform an analysis of the model's performance, including an examination of its word and character embeddings. 
% We observe that the model captures phonetic features, as evidenced by its use of character ngrams as input. 
% We also conduct language-wise and length-wise analyses to identify where errors occur and to understand why they happen.
We also perform a language-wise analysis, identifying which languages are most commonly confused by the model and explaining the reasons for these errors. We find that the model is biased towards IndicXlit, as the synthetic training data was generated using this model. Finally, we perform a length-wise analysis, showing that as the length of the input increases, the model's predictions become more stable and accurate. 
Overall, this work presents a comprehensive approach to Roman language identification for Indian languages, including the creation of a benchmark test set, a novel model, and detailed analysis of the model's performance and limitations.

% Overall, our work presents a novel approach to Roman language identification for Indian languages and provides valuable insights into the performance of this model.  Our findings provide valuable insights into the performance of this model and highlight its potential for use in natural language processing tasks.








\section{related work}
\textbf{work done on Roman inputs}\\
\textbf{LID models}\\
"LangID in wild" proposed a combine method of two techniques: wordlist-based tunable-precision filters and transformer-based semi-supervised LangID models. \\

\textbf{LID dataset and work done on Indian languages}\\

The related work section for a language identification model for Indian languages would likely include a discussion of previous research and existing approaches to language identification in general, as well as any existing models or techniques specifically designed for Indian languages. This section could also include a brief overview of the linguistic diversity of India, and the challenges and opportunities that this presents for language identification. Additionally, the related work section could discuss any relevant background information on the specific Indian languages that the model is designed to identify, such as their unique characteristics and features.\\

1. language Id in wild summary 
2. NLLB- LID model
3. Survey paper on LID and LID on Indian Languages
4. fasttext 5 paper on modeling
5. CLD3 model
5. list out all the papers with simple methods used in LID but before 2015. \\

6. fasttext model 5 paper, as in application of fasttext model in wide domain and justify how it is light weight, useful and effective. \\
7. recent and popular LID paper and show how your work is different or related/aligned from those papers.  \\
8. LID paper/work done on Indian languages \\






\section{Data creation}
\subsection{test set creation and filtration of Dakshina test set}
There is currently no benchmark test set available to evaluate Roman language identification in Indian languages. The Dakshina test set, which was originally created for language modeling, consists of parallel native and Roman sentences. However, this test set includes named entities and English loan words that can be pronounced the same across all languages, leading to confusion for the LID model in identifying the language. We have filtered out these corrupted inputs from the Dakshina test set. The process of filtering the test set is explained in Section \ref{subsubsec:dak_valid}.

% There is no benchmark test set available for Roman language identification task. Dakshina test set consists of parallel native and roman sentences which they have originally created for language modeling task. Those sentences could be of named entities, English loan words, or some unknown phrases (e.g.). Named entities and English loan words can be pronounced same across all the languages and therefore, their roman transliteration would be written same in all the languages. So, those phrases are really not needed in the test set or even create confusion for the LID model to identify its language. We take up this task to filter out those corrupted inputs from the test set. section \ref{subsubsec:dak_valid} explains the process of filtering the Dakshina test set.

\subsubsection{The process of validating Dakshina test set} \label{subsubsec:dak_valid}
We asked language annotators to validate the sentences by providing them with guidelines. The annotators were asked to read the phrases in Roman transliteration and determine whether the phrases belonged to the particular language. If the phrases were named entities or loan words from English, they would be written the same in Roman transliteration for all languages and should be marked as invalid sentences (1). Sentences that belonged to the particular language were marked as valid (0), while those that were confusing were marked as confused (2).
% We asked language annotators to validate the sentences. we provided some guidelines for the task. following are the guidelines, 
% \item \textbf{1.} mark 1 (invalid) if sentence or phrase does not belong to the particular language. we asked annotators the read the phrase in the roman transliteration and judge whether that phrase belong to the particular language. if it's named entity or loan words from english then those would be written same in roman transliteration  for all the languages. so those should be marked ass invalid sentences. 
% \item \textbf{2.} mark 0 (valid) if sentence or phrase belong to the particular language
% \item \textbf{3.} mark 2 (confused) if sentence or phrase is bit confusing and annotators is not able to identify it's language by  reading it.
\subsubsection{The process of creating benchmark test set for roman LID in all languages}
\subsection{Training data creation process}
\subsubsection{Indic-En IndicXlit model}
\refer{Aksharantar paper} released a multilingual transliteration model in En-Indic direction that is state-of-the-art for transliteration in Indian languages. We train the Indic-En model using the Aksharantar train data with the same model architecture described in the paper. It is multilingual character level transliteration model \cite{kunchukuttan-etal-2021-large} in a many-to-one setting, which consumes an Indic character sequence (Native script) and generates an output character sequence in the romanized language script. The output sequence includes a special \todo{\textit{source language tag}} token to specify the source language \cite{johnson17}. The input vocabulary is the union of characters from various Indic language scripts found in the training set, while the output vocabulary is the set of Roman characters found in the training set. The input and output vocabulary sizes are 780 and 28 characters, respectively. All other settings were same as IndicXlit model introduces in \ref{Aksharantar paper}. We report the results of IndicXlit Indic-En model on the Aksharantar and Dakshina testset in Table \ref{tab:rescoring_results}.
% \indent - table of results on Ak-test set (which is compiled set of Ak-test set and Dakshina test set) \\
\subsubsection{train data transliteration}
we collected various sources of data to create our training dataset. To ensure a diverse and representative sample, we selected a maximum of 1 million samples from each source. These samples were then collated and a random subset of 1 million samples was selected from the combined group. In cases where a particular language had fewer than 1 million samples, we used resampling techniques to duplicate the samples and reach the desired sample size of 1 million. This approach allowed us to create a balanced and comprehensive training dataset for our analysis.
% we have collated all the sources to create the training data. we take at most 1 M samples from each source, collate them and then take 1 M random sample from all the collated samples. we do the resamling if any lanaguge has less than 1 M samples. for resampling we just duplicate the samples. we resample upto 1 M samples.
\textbf{IndicCorp}: detail of IndicCorp paper in concise way\\
\textbf{NLLB} \\
\textbf{Wikidata} A Wikipedia dump is a complete and uncompressed copy of all of the articles, templates, images, and other data from a particular language edition of Wikipedia. These dumps are typically produced by the Wikimedia Foundation on a regular basis, and are available for download from their website. it is a valuable resource and it's large collection of Wikipedia articles. The WikiExtractor tool can be used to process these dumps and extract the articles and other data from them, in order to convert the raw data into a more usable format.\\
\textbf{Vikaspedia} Vikaspedia is an online information guide launched by the Government of India. The website was implemented by C-DAC Hyderabad and is run by the Department of Electronics and Information Technology, Ministry of Communications and Information Technology. It is built as a portal for the social sectors, and offers information in 23 languages. \\
\textbf{Manual samples} We collected number-k manual samples for some low resource languages. \viz. (list of languages) \\
\textbf{collation of all the sources} (100k samples with resampling technique(explain)) : table of stats describing the samples from each source. \\
\textbf{transliteration of all the sources via Indic-En IndicXlit model}: Preprocessing of text data (indic tokenization). we use the multilingual transliteration model described in section \ref{}  to transliterate all the native collated text to roman text. \\










\section{Experimentation/Ablation study (or more on "how we come up with the choices we made to achieve the benchmark results")}
we conducted a series of experiments to evaluate different design choices for our model. 
\subsection{2-stage model}
After careful consideration, we decided to use a two-stage approach that combines the strengths of different models. The first stage of the model uses fasttext, a lightweight linear classifier that is fast and efficient, but may not be as accurate as more complex models. The second stage of the model is IndicBERT, a more powerful language model that has been pre-trained on a large corpus of Indian language data. To make this model suitable for our classification task, we added a softmax classification layer at the end, which allows the model to predict the likelihood of each class.
Overall, our design choice allows us to achieve a good balance between speed and accuracy. The fasttext model provides quick and reliable predictions, while the IndicBERT model can refine and improve these predictions using its more sophisticated language modeling capabilities. By using a two-stage approach, we are able to take advantage of the best qualities of both models, resulting in an efficient and effective solution for our task.
% we have experimented lot of variation and come up with the following design choice. we use the 2 stage model which is a combination of a (i) lightweight model fasttext, a linear classifier model and (ii) a more powerful model IndicBERT, language model with added softmax classification layer added at the end of the model. 
% - explain and describe the details related to experimentation of each model individually.\\
\input{Table_fasttext_with_different_dimension_unclean}
\subsubsection{fasttext}
FastText is a library for efficient learning of word representations and sentence classification. It was developed by Facebook's AI Research lab (FAIR). It is particularly useful for handling large-scale text data, since it uses a hierarchical structure to represent words, which allows it to model the internal structure of words and to learn sub-word information. This makes it efficient for dealing with rare words and allows it to achieve good performance on a wide variety of tasks, such as language modeling, text classification. We have train fasttext model using 100k samples. Table \ref{tab:fasttext_with_different_dimension_unclean} describes the result of experiments done with the different dimension of fasttext model. \\
Write the model parameters and training details.
% brief about fasttext model, results on fasttext model \\
\input{Table_IndicBERT_finetuning_unfreezing_different_layers}
\subsubsection{Language model + linear layer (softmax 20 class) }
To fine-tune the language model, we added one softmax layer to the end of the model and used our training data. We experimented with three different pre-trained language models: IndicBERT, XLM-R, and MuRIL. In the initial experiment, we froze all the layers except for the last softmax layer and fine-tuned the model with our training data. We found that IndicBERT performed the best among these three models for our task. We then further experimented with IndicBERT by unfreezing 1, 2, 4, 6, 8, and 11 layers. The results and comparison of all the experiments are described in Table \ref{tab:IndicBERT_finetuning_unfreezing_different_layers}. We found that unfreezing only 1 layer was enough for our task and that unfreezing more layers did not provide any additional benefit.
% We finetune the language model with adding one softmax layer at the end of the model with our train data. we experiment with 3 different pretrianed language model. \viz IndicBERT, XLM-R, MuRIL. Intial experiment we freeze all the layers except for the last softmax layer and finetune the model with our training data. we found IndicBERT to the best among these three models for our task. We then further experiment with IndicBERT by unfreezing 1, 3, 5, 7, 11 layers. Table \refer{} describes the results and comparison of all the experiments. we found out that unfreezing 1 layer is enough for our task. unfreezing more layers do not give more benifit.  
% explain the study we have done on different model and finetune by unfreezing and then after selecting IndicBERT we again some sort of finetuning with unfreezing different layers \\
% table to compare all the experiments we did with language model \\
% results on IndicBERT model \\
\subsubsection{combination of 2 stage model}
we have described a two-stage model that combines the fasttext and IndicBERT models. The fasttext model, which is described in section \ref{}, is a light weight model that takes very little time for inference. On the other hand, the IndicBERT model, which we have seen in section \ref{}, is a more powerful model that takes more time for inference than the fasttext model. In order to take advantage of both models, we have designed a two-stage model.
In this model, we first give the input to the fasttext model. If the prediction score is greater than 0.8, we consider the output from the fasttext model as the final output. However, if the prediction score is less than 0.8, we back off to the IndicBERT model and consider the output from the IndicBERT model as our final output. This way, if the fasttext model is confident about the predicted language of the given text, we get the final output with less inference time. But if the fasttext model is not confident about the prediction, we back off to the more powerful IndicBERT model and maintain the accuracy of the overall model. The results we obtained from the two-stage model are shown in Table \ref{}.
% fasttext model describe in section \refer{} is light weight model and take very less time for inference whereas IndicBERT is very powerful model as we already seen in section \refer{} is heavy weight model and takes more time for inference than fasttext. To take the advantage of both model we design 2 stage model. we first give input to fasttext model if prediction score is greater than 0.8 we consider the output from fasttext model and if prediction score less than 0.8 we back off to IndicBERT model and consider the output from IndicBERT model as our final output. In other model if fasttext model is confident about the predicted language of the given text then we get the final output with less inference time but if fastext model is not confident about the predictino then we backoff to more powerful model and maintain the accuracy of overall model. Table \refer{} the result we got from 2 stage model.
% explain the model, diagram, how we incorporated using some threshold \\
% results on combine model, justifying that reducing the inference time with imporving the accuracy as well. \\
% different experiments can be shown in the table as in each column for techniques and improvements we got.

\subsection{Dataset cleaning: used native model}
we have performed a detailed analysis of the training data. Upon manual inspection, we found that there was a significant amount of noise and incorrect data in the corpus. This was particularly true for the language corpora in IndicCorp, where some of the text consisted of other languages. In order to improve the quality of the training data, we trained a native LID model using the available native script train data. This model allowed us to filter out any sentences that were not in the target language.
We set a threshold of 0.8 for the prediction score of a valid sentence, and discarded all sentences that were predicted with a score below 0.8. This helped us to identify and remove any sentences that were not in the target language, resulting in a cleaner and more accurate training set. We then transliterated this clean train data using the method described in section \ref{}. 
The results of the model trained with this clean train set are shown in Table \ref{}. As we can see from the table, the model achieved significantly better performance when trained on the cleaned and transliterated data, compared to the original training data. 
% We analyze the training data manually and observed that there was a lot of noise in the training data. Some language corpora in IndicCorp consist of other language text. We train the native LID model using the available native script train data and then use that model to filter the training data in the native script. we keep the threshold as 0.8 for the prediction score of the valid sentence. All the sentences that were predicted with prediction scores below 0.8 are invalid, and we discarded those sentences from the training data. Now, we again transliterate this train data same as method describe in section \refer{}. Table \ref{} shows the results of the model trained with this clean train set. 
% explain the issue and process of cleaning the process.\\
% table to show how it improved by just cleaning the data \\
% results of individual model as well as 2-stage model

\section{Result and Analysis}
\subsection{Results on IndicLID benchmark test set}
\subsection{Analysis}
we have performed an error analysis on the Dakshina Roman test set, which we have divided into four parts. The first part of our analysis focuses on the effectiveness of the word and character embeddings in capturing the linguistic features of the text. The second part of our analysis is a language-wise analysis, which allows us to evaluate the performance of our LID model to identifying which languages are most commonly confused by the model and explaining the reasons for these errors. The third part of our analysis is explaining the biaseness towards IndicXlit. Finally, we have also performed a length-wise analysis, which examines the performance of our model on text of different lengths.
The results of our error analysis are presented in detail in the following sections. Overall, our analysis has provided valuable insights into the strengths and weaknesses of our LID model, and has allowed us to identify areas for improvement. We plan to use these findings to refine our model and improve its performance on the Dakshina Roman test set.
% we have done a error analysis on the dakshina roman test set and categorized into 4 parts. 
\subsubsection{analysis of word embeddings or more of character embedding as in what it is capturing}
We have trained a skip-gram model provided by fasttext with our train data. This model allows us to generate word embeddings for our samples, which we can then use to identify the linguistic features that the embeddings are learning. In order to do this, we have used char-n-grams as our feature vector, and have measured the similarity between words using cosine similarity or word distance. Some examples of our analysis are shown in Table \ref{}.
From our analysis, we have observed that words with similar n-grams tend to be close to each other in the word embedding space. In other words, words that have some phonetic similarity tend to form clusters in the embedding space. This suggests that the word embedding model is effectively capturing the phonetic features of the text when we give the char-n-grams as input. Some examples of the n-grams or phonemes that we have identified are shown in Table \ref{}.
% we train a skip-gram model provided by fasttext with our train data. we generate the word embeddings of some samples to identify what embeddings are actually learning when we give the char-n-grams as our feature vector. We find the neighbour words given the sample word using cosine similarity or word distance. Some examples are shown in table \ref{}. We observe that words with similar n-grams are close to each other. In other words, words that have some phonetic similarity come together and form a cluster. Some examples of n-grams or phonemes are shown in table \ref{}. This analysis shows that word embedding model truly captures the phonetic feature of the given text when we give the char-n-grams as input to the model.

\subsubsection{language wise analysis}
We have observed that as we train our model on more languages, it becomes more prone to errors and confusion in identifying the languages. This can be seen in Table \ref{}, which shows a comparison of models trained on 9, 12, and 22 languages. We have also manually inspected some samples from the training data of similar languages, and have found that there are many instances of word overlap across languages. For example, some Hindi words such as "list of some examples" are found in the Nepali training data.
To further analyze this issue, we have calculated a confusion matrix of word overlaps across all the languages. The results of this analysis are shown in Table \ref{}, which shows the number of words that are overlapped across each language pair. From this table, we can see that languages that have a higher number of word overlaps are more likely to cause errors in the LID model. This is because the last linear layer of the fasttext LID model projects the sentence embedding into the embedding space/cluster of the particular language. If a Nepali sentence contains Hindi words, the LID model may project the Nepali sentence embedding into the Hindi embedding space/cluster, leading to confusion and errors.
To address this issue, we need to develop more robust and concrete features for identifying the language of a given sentence with overlapping words. This will require further research and experimentation, but is an important area for improving the performance of our LID model.
% We observe that as we train the model with more languages, it becomes more prone to errors and creates more confusion in identifying the languages. Table \ref{} shows the comparison of models trained in 9, 12, and 22 languages. We manually try to look at some samples from the training data of similar languages. for instance, these Hindi words \viz \textit{list of some examples} are found in Nepali training data. We calculated the confusion matrix of word overlaps across all the languages. table \ref{} shows the number of words overlapped across each and every language. We observe that, languages which have more word overlaps are more prone to create errors. This is quite evident because last linear of fasttext LID model projects the sentence embedding to the space/cluster of the particular language. If Nepali sentence contains Hindi words, then LID may project the particular sentence embedding to the space where the Hindi cluster lies. This can't be avoided. We need more strong/concrete features to identify the language given the sentence with overlapping words.
% among which languages the highest errors happen and explaining why it is the case via error analysis\\
% more languages creates more confusion because input is roman, table of LId model trained on 9, 12, 20 languages\\
% words are getting overlapped between similar languages, can be shown with word-overlaps stats in the table and with some examples.
\subsubsection{Also bit biased towards IndicXlit}
we have generated the train data using the IndicXlit Indic-En model. The IndicXlit model is a multilingual transliteration model that supports 20 Indian languages and is trained on character-level input. This means that it learns the interactions between characters while being trained on multiple language pairs.
However, the IndicXlit model has only seen a limited set of character ngrams (i.e. sequences of characters) during training. This means that when we transliterate the LID training data through IndicXlit, the resulting romanized text will only contain the character ngrams that were seen by the IndicXlit model. As a result, the roman LID model will only be able to learn to identify languages using a limited set of ngrams generated by the IndicXlit model.
When the Dakshina dataset is transliterated through IndicXlit, the resulting romanized version will only contain the character ngrams that were seen by the IndicXlit model. This means that the LID model will be able to accurately predict the language of sentences in the transliterated test set, as it will encounter only character ngrams that it has seen during training.
This creates a challenge for the LID model when it is applied to the original Dakshina roman test set. The model may encounter character ngrams that were not present in the training data, making it difficult for it to accurately predict the language of the sentence. 
Overall, this issue arises because the LID model is trained on synthetic data generated by a transliteration model, which may not capture the full range of character ngrams that are present in the real-world. As a result, the LID model may struggle to accurately predict the language of sentences that contain unseen character ngrams. This is evident from the results shown in Table \ref{}, which compares the accuracy of the LID model on the Dakshina original romanized text and the transliterated text of Dakshina native inputs using IndicXlit model. The marginal difference in accuracy between the two test sets indicates that to improve the performance of the LID model, we need to find ways to better handle the challenge posed by the IndicXlit model and its ability to generate a limited set of character ngrams.

% we have generated the train data using the IndicXlit Indic-En model. The IndicXlit model is a multilingual transliteration model that supports 20 Indian languages and is trained on character-level input. This means that it learns the interactions between characters while being trained on multiple language pairs.
% However, the IndicXlit model has only seen a limited set of character ngrams (i.e. sequences of characters) during training. So when we transliterate the LID training data through IndicXlit the romanized text will only contain the character ngrams that were seen by the IndicXlit model but not all the ngrams which could be in real-world. This happens same with the Dakshina test set. when the Dakshina dataset is transliterated through IndicXlit, the resulting romanized version will only contain the character ngrams that were seen by the IndicXlit model. Some character ngrams that are present in the Dakshina test set may not be present in the romanized version of the dataset. 

% we have generated the train data using the IndicXlit Indic-En model. The IndicXlit model is a multilingual transliteration model that supports 20 Indian languages, and is trained on character-level input. This means that it learns the interactions between characters while being trained on multiple language pairs. 
% IndicXlit model have seen some character ngrams and would not have seen some character ngrams. Now when Dakshina dataset is transliterated through IndicXlit romanized version would have all seen all the ngrams generated by IndicXlit model but some ngrams would not be present which is in real world or in Dakshina test set. 
% Based on the principles of multilinguality, we can expect that the IndicXlit model will transfer knowledge from high-resource languages to low-resource languages while training. In our case, this means that the model may use knowledge from Hindi (a high-resource language) while learning to transliterate Nepali (a low-resource language). 
% % Since the IndicXlit model is a character-level model, it  the same character n-grams to transliterate Nepali that it learned from Hindi.
% it may use the same character ngrams (i.e. sequences of characters) to represent some words in different languages. This means that if IndicXlit uses the same character ngrams to represent words in two different languages, the language identification model is relying on the same character ngrams to distinguish between them.
% This can cause confusion between similar languages because there is more chance of knowledge to be transferred between similar languages while training the IndicXlit model. 
% % because the LID model is relying on the same character ngrams to distinguish between them. 
% For example, Nepali is low resource language and Hindi is high resource language, There is one word which is very similar in Nepali and Hindi but its unseen while training. IndicXlit model will use the knowledge from Hindi while transliterating that word in Nepali (roman text) because it has similar ngrams and word is not present in Nepali. Now, that word vector will fall into Hindi embedding space    
% For example, if IndicXlit uses the same character ngrams to represent words in Hindi and Nepali, the language identification model will also use those same character ngrams to identify these languages. This can lead to errors in the model's predictions, as it may not be able to accurately distinguish between similar languages.
% Overall, this issue arises because the language identification model is using synthetic data generated by a transliteration model, which may not capture the unique characteristics of each language. As a result, the model may not be able to accurately identify languages that have similar characteristics.
% % This creates a challenge for the LID task, which is to identify the language of a given text that has been generated by a multilingual transliteration model. The LID model may be confused by the similarities between languages, leading to errors in its predictions. 
% This is evident from the results shown in Table \ref{}, which compares the accuracy of the LID model on the Dakshina original romanized text and the transliterated text of Dakshina native inputs using IndicXlit model. The marginal difference in accuracy between the two test sets indicates that the LID model is struggling to correctly identify the language of the original roman text. To improve the performance of the LID model, we need to find ways to better handle the challenge posed by the IndicXlit model and its ability to transliterate between languages.
% Overall, this issue arises because the language identification model is using synthetic data generated by a transliteration model, which may not capture the unique characteristics of each language. As a result, the model may not be able to accurately identify languages that have similar characteristics.
% When the model is trained using synthetic data generated by a multilingual transliteration model like IndicXlit, it uses the same character ngrams (i.e. sequences of characters) to represent some words in different languages. This means that if IndicXlit uses the same character ngrams to represent words in two different languages, the language identification model will also use those same character ngrams to identify those languages.
% This can cause confusion between similar languages because the model is relying on the same character ngrams to distinguish between them. For example, if IndicXlit uses the same character ngrams to represent words in Hindi and Punjabi, the language identification model will also use those same character ngrams to identify these languages. This can lead to errors in the model's predictions, as it may not be able to accurately distinguish between similar languages.
% Overall, this issue arises because the language identification model is using synthetic data generated by a transliteration model, which may not capture the unique characteristics of each language. As a result, the model may not be able to accurately identify languages that have similar characteristics.
% We generate the train data using IndicXlit Indic-En model. Now, IndicXlit model is multilingual in nature and it's a single model that supports 20 Indian languages. from the study of multilinguality we can say that multilingual model transfers the knowledge from high resource language to low resource language while training with multiple pairs across languages. Also IndicXlit model is character level model. So, it learns the interaction between characters while we train it. therefore IndicXlit model might used the knowledge from Hindi (Hing resource language) while learning for Nepali (low resource language). And since it is character level model it is using the same character n-grams to transliterate Nepali which is learned from character n-grams of Hindi. Now, LID task is to identify the language given the text that is generated through the multilingual model which is bit contrary in nature. This justifies the confusion created by LID model across similar language. Table \refer{} shows the accuracy on Dakshina original romanized text and trasnliterated text of Dakshina native inputs. This is quite  evident from the marginal difference of accuracy between two test set.
% as synthetic train data generated using IndicXlit \\
% IndicXlit transfer the knowledge across languages when it was trained, specifically from high to low-resource languages. it also depends on character-level information.\\ 
% So while transliterating low-resource language, it might be using the same char n-grams as it learned from high-resource languages (it might be using the same n-grams to transliterate low resource which it is uses to transliterate high resource languages). \\
% Now, we are distinguish the language using the same phonetic characterisitc or so to say same char ngrams. \\
% this is evident when we evalute the model with Dakshina romanzied through IndicXlit and original Dakshina roman inputs

\subsubsection{Length wise analysis}
we have divided the test set into different buckets according to the length of the sentences. We have performed our analysis on the 3-length and 5-length buckets, and have observed that as the length of the sentence increases, the model is able to predict the correct language with higher confidence. This is an intuitive result, as providing more information to the model about a particular sentence should allow it to make a more accurate prediction.
The results of our analysis are shown in Table \ref{}, which compares the accuracy of the LID model on the 3-length and 5-length buckets of the test set. As we can see from the table, the accuracy of the model increases as the length of the sentences in the test set increases. This demonstrates the importance of providing sufficient information to the LID model in order to improve its performance.
% we divide the test set into the different buckets according to their length. we have analyzed 3-length bucket and 5-length buckets. we observe that as the length of the sentence increases model predicts the correct language with higher confidence. This is quite intutive as in if we give more information to the model for a particular sentence, model predicts the language with higher confidence. Table \ref{} shows the accuracy for 5 length buckets and 3 length buckets. 
% As we increase the length prediction gets more stable and accuracy improves. It is quite obivious as model would have more information to evalute the sentence to identify it's language.\\
% 5 len bucket, \\
% 3 len bucket
\section{Conclusion}


==> Table_7_9_11_22_languages_f1_precision_recall_roman.tex <==
% \newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}
\begin{table*}[t]
% \setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{1.3}
    \centering
    % \fontsize{10}{12}
    \scalebox{0.80}{
    \begin{tabular}{l|rrr|rrr|rrr|rrr}
     \toprule
     &\multicolumn{3}{c|}{7 languages} &\multicolumn{3}{|c|}{9 languages} &\multicolumn{3}{|c|}{11 languages} &\multicolumn{3}{|c}{22 languages} \\
     \midrule
     &Precision &Recall &F1 &Precision &Recall &F1 &Precision &Recall &F1 &Precision &Recall &F1 \\
     \midrule
    Assamese &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.72 &0.93 &0.81 \\
    Bangla &0.95 &0.99 &0.97 &0.96 &0.98 &0.97 &0.91 &0.98 &0.95 &0.95 &0.94 &0.94 \\
    Bodo &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.86 &0.99 &0.92 \\
    Konkani &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.41 &0.98 &0.58 \\
    Gujarati &0.95 &0.95 &0.95 &0.94 &0.93 &0.94 &0.93 &0.93 &0.93 &0.95 &0.87 &0.91 \\
    Hindi &0.99 &0.93 &0.96 &0.96 &0.89 &0.92 &0.71 &0.82 &0.76 &0.77 &0.53 &0.63 \\
    Kannada &0.96 &0.98 &0.97 &0.95 &0.97 &0.96 &0.91 &0.98 &0.94 &0.95 &0.97 &0.96 \\
    Kashmiri &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.35 &0.95 &0.51 \\
    Maithili &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.22 &0.44 &0.29 \\
    Malayalam &0.96 &0.97 &0.96 &0.93 &0.97 &0.95 &0.9 &0.98 &0.94 &0.91 &0.95 &0.93 \\
    Manipuri &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.59 &0.99 &0.74 \\
    Marathi &0 &0 &0 &0.95 &0.89 &0.92 &0.94 &0.9 &0.92 &0.96 &0.83 &0.89 \\
    Nepali &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.37 &0.94 &0.53 \\
    Oriya &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.63 &0.97 &0.76 \\
    Punjabi &0 &0 &0 &0.89 &0.94 &0.91 &0.82 &0.91 &0.86 &0.86 &0.63 &0.72 \\
    Sanskrit &0 &0 &0 &0 &0 &0 &0 &0 &0 &0.37 &0.99 &0.54 \\
    Sindhi &0 &0 &0 &0 &0 &0 &0.86 &0.82 &0.84 &0.88 &0.73 &0.79 \\
    Tamil &0.97 &0.97 &0.97 &0.95 &0.97 &0.96 &0.97 &0.96 &0.96 &0.98 &0.93 &0.95 \\
    Telugu &0.95 &0.94 &0.94 &0.93 &0.93 &0.93 &0.95 &0.92 &0.93 &0.96 &0.89 &0.93 \\
    Urdu &0 &0 &0 &0 &0 &0 &0.81 &0.48 &0.61 &0.87 &0.46 &0.6 \\
    \midrule
    Avg &0.96 &0.96 &0.96 &0.94 &0.94 &0.94 &0.88 &0.88 &0.88 &0.73 &0.85 &0.75 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{Precision, recall and F1-score of \modelname roman script model trained with different number of languages. All scores are calculated on \dsname roman script test set}
    \label{tab:Table_7_9_11_22_languages_f1_precision_recall_roman}
    % \vspace{-4mm}
\end{table*}

==> Table_Bhasha_Abhijnaanam_stats_in_detail.tex <==
% \newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}
\begin{table*}[t]
% \setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{1.3}
    \centering
    % \fontsize{10}{12}
    \scalebox{0.80}{
    \begin{tabular}{l|rrrrr|rrrr}
     \toprule
     &\multicolumn{5}{c|}{Native script test set} &\multicolumn{4}{|c}{Roman script test set} \\
     \midrule
    Language &Dakshina &Flores &AI4B &Total 
    &Deduplicates &Dakshina &Benchmark &Total &Deduplicates \\
     \midrule
    Assamese &0 &1012 &0 &1012 &1012 &0 &512 &512 &512 \\
    Bangla &4600 &1012 &0 &5612 &5606 &4600 &0 &4600 &4595 \\
    Bodo &0 &0 &1500 &1500 &1500 &0 &433 &433 &433 \\
    Dogri &0 &0 &1500 &1500 &1498 &0 &0 &0 &0 \\
    Gujarati &4789 &1012 &0 &5801 &5797 &4789 &0 &4789 &4785 \\
    Hindi &4616 &1012 &0 &5628 &5617 &4616 &0 &4616 &4606 \\
    Kannada &4849 &1012 &0 &5861 &5859 &4849 &0 &4849 &4848 \\
    Kashmiri-Arab &0 &1012 &1500 &2512 &2511 &0 &450 &450 &450 \\
    Kashmiri-Deva &0 &1012 &0 &1012 &1012 &0 &0 &0 &0 \\
    Konkani &0 &0 &1500 &1500 &1500 &0 &444 &444 &444 \\
    Maithili &0 &1012 &1500 &2512 &2512 &0 &439 &439 &439 \\
    Malayalam &4627 &1012 &0 &5639 &5628 &4627 &0 &4627 &4617 \\
    Manipur-Mei &0 &0 &1500 &1500 &1500 &0 &442 &442 &442 \\
    Manipuri-Beng &0 &1012 &0 &1012 &1012 &0 &0 &0 &0 \\
    Marathi &4617 &1012 &0 &5629 &5611 &4617 &0 &4617 &4603 \\
    Nepali &0 &1012 &1500 &2512 &2512 &0 &423 &423 &423 \\
    Oriya &0 &1012 &0 &1012 &1012 &0 &512 &512 &512 \\
    Punjabi &4782 &1012 &0 &5794 &5776 &4782 &0 &4782 &4765 \\
    Sanskrit &0 &1012 &1500 &2512 &2510 &0 &448 &448 &448 \\
    Santali &0 &1012 &1500 &2512 &2512 &0 &0 &0 &0 \\
    Sindhi &4889 &1012 &0 &5901 &5893 &4889 &0 &4889 &4881 \\
    Tamil &4802 &1012 &0 &5814 &5779 &4802 &0 &4802 &4767 \\
    Telugu &4754 &1012 &0 &5766 &5751 &4754 &0 &4754 &4741 \\
    Urdu &4395 &1012 &1500 &6907 &6883 &4395 &0 &4395 &4371 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{Detailed statistics of \dsname testset}
    \label{tab:Table_Bhasha_Abhijnaanam_stats_in_detail}
    % \vspace{-4mm}
\end{table*}

==> Table_Fasttext_Cld3_Nllb_f1_precision_recall_native.tex <==
% \newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}
\begin{table*}[t]
% \setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{1.3}
    \centering
    % \fontsize{10}{12}
    \scalebox{0.80}{
    \begin{tabular}{l|rrr|rrr|rrr}
     \toprule
     &\multicolumn{3}{c|}{\modelnamefasttextnative(24)} &\multicolumn{3}{|c|}{CLD3 model (12)} &\multicolumn{3}{|c|}{NLLB model(20)} \\
     \midrule
     &Precision &Recall &F1 &Precision &Recall &F1 &Precision &Recall &F1 \\
     \midrule
    Assamese &0.97 &1 &0.98 &0 &0 &0 &1 &1 &1 \\
    Bangla &1 &0.99 &1 &1 &1 &1 &1 &1 &1 \\
    Bodo &0.99 &0.99 &0.99 &0 &0 &0 &0 &0 &0 \\
    Dogri &0.99 &0.96 &0.97 &0 &0 &0 &0 &0 &0 \\
    Konkani &0.97 &0.99 &0.98 &0 &0 &0 &0 &0 &0 \\
    Gujarati &1 &1 &1 &1 &1 &1 &1 &1 &1 \\
    Hindi &0.96 &0.92 &0.94 &0.96 &0.96 &0.96 &0.94 &0.98 &0.96 \\
    Kannada &1 &1 &1 &1 &1 &1 &1 &1 &1 \\
    Kashmiri\_Arab &0.97 &0.99 &0.98 &0 &0 &0 &1 &0.96 &0.98 \\
    Kashmiri\_Deva &0.96 &0.96 &0.96 &0 &0 &0 &1 &0.97 &0.98 \\
    Maithili &0.81 &0.93 &0.87 &0 &0 &0 &0.99 &0.93 &0.96 \\
    Malayalam &1 &1 &1 &1 &1 &1 &1 &1 &1 \\
    Manipuri\_Beng &1 &1 &1 &0 &0 &0 &1 &1 &1 \\
    Manipuri\_Mei &1 &1 &1 &0 &0 &0 &0 &0 &0 \\
    Marathi &0.99 &0.96 &0.97 &0.97 &0.94 &0.95 &0.99 &0.96 &0.97 \\
    Nepali &0.98 &1 &0.99 &0.91 &0.99 &0.95 &0.97 &1 &0.98 \\
    Oriya &1 &1 &1 &0 &0 &0 &1 &1 &1 \\
    Punjabi &1 &1 &1 &1 &1 &1 &1 &1 &1 \\
    Sanskrit &0.98 &1 &0.99 &0 &0 &0 &1 &0.98 &0.99 \\
    Santali &1 &1 &1 &0 &0 &0 &1 &1 &1 \\
    Sindhi &0.99 &1 &0.99 &0.99 &0.96 &0.98 &1 &0.98 &0.99 \\
    Tamil &1 &1 &1 &1 &1 &1 &1 &1 &1 \\
    Telugu &1 &1 &1 &1 &0.99 &0.99 &1 &1 &1 \\
    Urdu &1 &0.98 &0.99 &1 &0.95 &0.97 &0.98 &0.98 &0.98 \\
    \midrule
    Avg &0.98 &0.99 &0.98 &0.99 &0.98 &0.98 &0.99 &0.99 &0.99 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{Precision, recall and F1-score of \modelnamefasttextnative, Cld3 and NLLB native script model. All scores are calculated on \dsname native script test set}
    \label{tab:Table_Fasttext_Cld3_Nllb_f1_precision_recall_native}
    % \vspace{-4mm}
\end{table*}

==> Table_IndicBERT_MuRiL_unfreeze_1_f1_precision_recall_roman.tex <==
% \newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}
\begin{table*}[t]
% \setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{1.3}
    \centering
    % \fontsize{10}{12}
    \scalebox{0.80}{
    \begin{tabular}{l|rrr|rrr}
    &\multicolumn{3}{|c|}{IndicBERT (unfreeze 1)} &\multicolumn{3}{c}{MuRiL (unfreeze 1)} \\
     \midrule
     &Precision &Recall &F1 &Precision &Recall &F1 \\
     \midrule
    Assamese &0.67 &0.91 &0.77 &0.75 &0.9 &0.82 \\
    Bangla &0.97 &0.88 &0.92 &0.94 &0.93 &0.94 \\
    Bodo &0.85 &0.99 &0.91 &0.73 &1 &0.84 \\
    Konkani &0.38 &0.99 &0.55 &0.55 &0.91 &0.69 \\
    Gujarati &0.96 &0.85 &0.9 &0.98 &0.85 &0.91 \\
    Hindi &0.76 &0.6 &0.67 &0.74 &0.65 &0.7 \\
    Kannada &0.96 &0.96 &0.96 &0.95 &0.96 &0.95 \\
    Kashmiri &0.39 &0.93 &0.55 &0.32 &0.88 &0.47 \\
    Maithili &0.29 &0.42 &0.34 &0.15 &0.49 &0.23 \\
    Malayalam &0.92 &0.95 &0.94 &0.92 &0.95 &0.94 \\
    Manipuri &0.5 &0.98 &0.66 &0.47 &0.98 &0.63 \\
    Marathi &0.96 &0.81 &0.88 &0.94 &0.83 &0.88 \\
    Nepali &0.43 &0.94 &0.59 &0.57 &0.97 &0.72 \\
    Oriya &0.64 &0.96 &0.77 &0.56 &0.97 &0.71 \\
    Punjabi &0.85 &0.65 &0.73 &0.9 &0.84 &0.87 \\
    Sanskrit &0.33 &0.99 &0.49 &0.38 &0.96 &0.54 \\
    Sindhi &0.86 &0.72 &0.78 &0.88 &0.58 &0.7 \\
    Tamil &0.97 &0.93 &0.95 &0.98 &0.94 &0.96 \\
    Telugu &0.95 &0.89 &0.92 &0.97 &0.87 &0.92 \\
    Urdu &0.89 &0.45 &0.6 &0.78 &0.5 &0.61 \\
    Avg &0.73 &0.84 &0.75 &0.72 &0.85 &0.75 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{Precision, recall and F1-score of IndicBERT and MuRiL roman script model. All scores are calculated on \dsname roman script test set}
    \label{tab:Table_IndicBERT_MuRiL_unfreeze_1_f1_precision_recall_roman}
    % \vspace{-4mm}
\end{table*}

==> Table_IndicXlit_Indic_En_results.tex <==
% \newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}
\begin{table*}[]
% \setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.4}
    \centering
    % \fontsize{10}{12}
    \scalebox{0.58}{
    \begin{tabular}{lrrrrrrrrrrrrrrrrrrrr}
    \toprule
        \textbf{Testset} 
          &\textbf{asm} &\textbf{ben} &\textbf{brx} &\textbf{guj} &\textbf{hin} &\textbf{kan} &\textbf{kas} &\textbf{kok} &\textbf{mai} &\textbf{mal} &\textbf{mni} &\textbf{mar} &\textbf{nep} &\textbf{ori} &\textbf{pan} &\textbf{san} &\textbf{tam} &\textbf{tel} &\textbf{urd} &\textbf{avg} \\
    \midrule
    % \multicolumn{21}{l}{} \\
    \textbf{AK-Freq} &76.9 &10.8 &72.09 &41.31 &39.5 &51.09 &79.4 &57.35 &81.746 &70.1 &84.64 &45.4 &85.27 &55.5 &29.9 &69.6 &55.64 &63.1 &- &59.40 \\
    \textbf{AK-Uni} &74.2 &12.71 &65.02 &36.6 &29.2 &53.5 &73.1 &54.22 &48.2 &61.00 &- &26.9 &79.5 &51.8 &28.2 &65.2 &34.5 &46.00 &29.95 &48.32 \\
    \textbf{AK-NEF} &33.91 &45.46 &28.96 &26.97 &44.7 &53.23 &53.55 &06.63 &28.14 &40.07 &26.4 &49.75 &46.28 &42.02 &41.00 &39.44 &34.10 &52.70 &19.27 &37.50 \\
    \textbf{AK-NEI} &40.39 &57.03 &39.66 &40.61 &54.46 &63.31 &65.63 &17.12 &45.02 &48.79 &40.72 &61.36 &59.37 &51.53 &52.80 &44.95 &36.37 &60.94 &25.75 &47.67 \\
    \midrule
    \textbf{Micro-avg} &57.40 &49.75 &52.45 &36.98 &57.62 &62.42 &76.26 &33.75 &51.70 &64.13 &59.09 &62.04 &68.28 &50.41 &51.77 &53.94 &55.15 &63.83 &41.02 &55.16 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Top-1 accuracy for IndicXlit on various multi-reference testsets.}
    \label{tab:Table_IndicXlit_Indic_En_results}
    \vspace{-4mm}
\end{table*}

==> Table_language_wise_analysis_roman.tex <==

\begin{table}[]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{l|rrrr}
    \toprule
    \textbf{Trained on} &\textbf{Precision} &\textbf{Recall} &\textbf{F1-Score} &\textbf{Accuracy} \\  
    \midrule
    7 languages &0.96 &0.96 &0.96 &96.04 \\
    9 languages &0.94 &0.94 &0.94 &94.15 \\
    11 languages &0.88 &0.88 &0.88 &88.2 \\
    22 languages &0.73 &0.85 &0.75 &80.4  \\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparing results of models trained on different languages}
    \label{tab:Table_language_wise_analysis_roman}
\end{table}

